ActiveEA: Active Learning for Neural Entity Alignment

Entity Alignment (EA) aims to match equivalent entities across different Knowledge Graphs (KGs) and is an essential step of KG fusion. Current mainstream methods -- neural EA models -- rely on training with seed alignment, i.e., a set of pre-aligned entity pairs which are very costly to annotate. In this paper, we devise a novel Active Learning (AL) framework for neural EA, aiming to create highly informative seed alignment to obtain more effective EA models with less annotation cost. Our framework tackles two main challenges encountered when applying AL to EA: (1) How to exploit dependencies between entities within the AL strategy. Most AL strategies assume that the data instances to sample are independent and identically distributed. However, entities in KGs are related. To address this challenge, we propose a structure-aware uncertainty sampling strategy that can measure the uncertainty of each entity as well as its impact on its neighbour entities in the KG. (2) How to recognise entities that appear in one KG but not in the other KG (i.e., bachelors). Identifying bachelors would likely save annotation budget. To address this challenge, we devise a bachelor recognizer paying attention to alleviate the effect of sampling bias. Empirical results show that our proposed AL strategy can significantly improve sampling quality with good generality across different datasets, EA models and amount of bachelors.

==> sections/note.tex <==

\section{Baselines, variants or explorative methods}
\todo{This section will be put in appendix part.}

\subsection{Random Selection}
This is used as one baseline. The order to selected entities is random.

\subsection{Topology-based Heuristics}

\subsubsection{Degree}
The degree of a certain entity $e$ in KG is used as its acquisition function.
$$f^{ac}(e)=\mathrm{degree}(e)$$

\subsubsection{Pagerank}
In pagerank, the nodes with larger degree is more important. In addition, when two entities have the same degrees, the one connected with more important neighbours is thought more important.
$$f^{ac}(e)=\mathrm{pagerank}(e | \mathcal{G})$$

\todo{
    TODO: 
    consider other graph variants inputed to pagerank: 1) replace the directed edges with their corresponding inverse ones, 2) create two edges of two directions for each edge.
}


\subsection{Uncertainty-based Heuristics.}
For a certain entity $e$, the EA model can predict its matching scores $\mathbf{s}=\{s(e'_i|e)\}$ with every unlabelled entities in another KG. We can normalize the scores and use the normalized scores as the probabilities $\mathbf{p}_e=\{p(e'_i|e)\}$. 
There are many measures of uncertainty in existing works. We consider the following ones.

\subsubsection{Max Entropy}
$$f^{ac}(e)=\mathcal{H}(\mathbf{p}_e)=-\sum_{i=1} p(e'_i|e) \log p(e'_i|e)$$

\subsubsection{Least confidence}
$$f^{ac}(e)=1 - \max p(e'_i|e)$$

\subsubsection{Smallest Margin}
$$f^{ac}(e)=p(e'_*|e) - p(e'_{**}|e)$$ or 
$$f^{ac}(e)=s(e'_*|e) - s(e'_{**}|e)$$
where $e'_*$ is the entity with highest matching score while $e'_{**}$ is the one with the second highest score.


\subsection{Deep Uncertainty-based Heuristics.}
Deep Bayesian models have a parameter distribution $p(w)$ instead of a single deterministed parameter. So we usually sample several parameters from the distribution and do the predictions with them to get the scores $s(e'_i|e_i, w)$ or probababilities $p(e'_i|e_i, w)$. Then we calculate the expectation of the prediction results as the final prediction.
$$s(e'_i|e)=\mathbb{E}_{w \sim p(w)} s(e'_i|e, w)$$
$$p(e'_i|e)=\mathbb{E}_{w \sim p(w)} p(e'_i|e, w)$$
The traditional uncertainty-based heuristics can also be used for deep Bayesian models by replacing the probabilities or scores with the expected (mean) ones outputed by Bayesian models.
In addition, there are two special heuristics for deep bayesian model.
\subsubsection{BALD}
$$f^{ac}(e)=\mathbb{I}[\mathbf{p}_e, w] = \mathbb{H}[p(e'|e)] - \mathbb{E}_{\hat{w} \sim p(w)} [\mathbb{H}[p(e'|e, \hat{w})]]$$

\subsubsection{Standard Deviation}
$$\sigma_i (e) = \sqrt{\mathbb{E} [p(e'_i | e, w)^2] - \mathbb{E}_{q(w)} [p(e'_i | e, w)]^2 }$$
$$f^{ac}(e)=\sigma (e) = \frac{1}{N} \sum_i \sigma_i$$
where $N$ is the number of entities $e'$.




\subsection{Characteristics of EA Models}

\todo{TODO: Add a table to summarize the characteristics of EA models to support our selection of EA model.}






